Active Fairness Auditing

The fast spreading adoption of machine learning (ML) by companies across industries poses significant regulatory challenges. One such challenge is scalability: how can regulatory bodies efficiently audit these ML models, ensuring that they are fair? In this paper, we initiate the study of query-based auditing algorithms that can estimate the demographic parity of ML models in a query-efficient manner. We propose an optimal deterministic algorithm, as well as a practical randomized, oracle-efficient algorithm with comparable guarantees. Furthermore, we make inroads into understanding the optimal query complexity of randomized active fairness estimation algorithms. Our first exploration of active fairness estimation aims to put AI governance on firmer theoretical foundations.

==> new_separation.tex <==
\note{Tom: format the paper with the additional connections}

\begin{proposition}
There exists a hypothesis class and distribution $\Dcal_X$ over $\Xcal$ such that, for some $\epsilon > 0$ and $k$ the range of DP's of models in $\Hcal$: $|\mu(h) - \mu(h')| \leq k \epsilon$ $\forall h, h' \in \Hcal$ and $\CC(\Hcal) \leq O(\log 1 / \epsilon)$, but the complexity of active learning $h^*$ is $\Omega(d \log 1 / \epsilon)$ \note{Maybe change to $\Omega(d)$}.
\end{proposition}
%\chicheng{I think we don't need $k = o(1/\epsilon)$? We can allow $k = 1/\epsilon$?}

\chicheng{Overall I liked this example. On the other hand, it is brittle, in that if we change the hypothesis class to $\Hcal = \cbr{\sign(\inner{a}{x}): \|a\|_2 = 1}$, or $\Hcal = \cbr{ \sign(\inner{a}{x} +b): \| a \|_2 = 1, b \in \RR } = \cbr{ \sign(\inner{a}{x} + 1): a \in \RR^d }$, the same argument does not carry over..
}


\begin{proof}

We will analyze the following setting. Let $\Hcal = \{(a, 1): a \in \mathbb{R}^d, \|a\| = 1\}$, non-homogeneous linear classifiers with offset $1$. Define $\Dcal_X$ such that the conditional distribution $x \mid x_A = 1 \sim N(\mu_1, I)$, $\mu_1 = \alpha e_1$;  and $x \mid x_A = 0 \sim N(\mu_0, I)$, $\mu_0 = 0$.

Then, we have that for $h_a(x) = \inner{a}{x} + 1$:
\begin{align*}
    & \PP(h^*(x) = +1 \mid x_A = 1) - \PP(h^*(x)  = +1 \mid x_A = 0) \\
    & \qquad = \Phi(\alpha a_1 + 1) - \Phi(1)
\end{align*}
Since $\Phi(1 + \alpha) - \Phi(1 - \alpha)$ is monotonic, take $\alpha > 0$ to be the unique value such that $\Phi(1 + \alpha) - \Phi(1 - \alpha) = k\epsilon$. Note that $|a_1| \leq 1$ and thus $|\mu(h) - \mu(h')| \leq k \epsilon$ $\forall h, h' \in \Hcal$. Moreover, DP's extrema are attainable and attained at classifiers with $a_1 = \pm 1$.

Let $\mu_{\min} = \Phi(-\alpha + 1) - \Phi(1)$.  Since $\Phi(a_1 \alpha + 1) - \Phi(1)$ is increasing in $a_1$, there exists $k$ intervals over $a_1$, $[z_i, z_{i+1}]$ for $i \in [k]$ such that $\bigcup_{i \in [k]} [z_i, z_{i+1}] = [-1, 1]$ and $a_1 \in [z_i, z_{i+1}] \Leftrightarrow \Phi(a_1 \alpha + 1) - \Phi(1) \in [\mu_{\min} + i\epsilon, \mu_{\min} + (i + 1) \epsilon]$. Auditing requires determining the interval $i$ that $\mu(h^*)$ belongs to: $[\mu_{\min} + i\epsilon, \mu_{\min} + (i + 1) \epsilon]$, or equivalently the interval $[z_i, z_{i+1}]$ $a_1$ belongs to.

We will show that binary search can do this efficiently. Binary search may be implemented as follows:
\begin{itemize}
    \item When $c > 0$, to test if $a_1 \geq c$, deploy $x = -1 / c e_1$. A negative label for $x$ confirms this because $-a_1/c + 1 \leq 0 \Leftrightarrow a_1/c \geq 1 \Leftrightarrow a_1 \geq c$.
    \item When $c < 0$, to test if $a_1 \geq c$, deploy $x = -1 / c e_1$. A positive label for $x$ confirms this because $-a_1/c + 1 \geq 0 \Leftrightarrow 1 \geq a_1 / c \Leftrightarrow c \leq a_1$.
\end{itemize}

%\chicheng{This seems only work when $c < 0$, and we need to also handle the cases when $c = 0$ and $c > 0$?} 

Using binary search we may find $\max\cbr{i: z_i \leq a_i}$ over the $k+1$ numbers. We note that our midpoint check only applies for when $z_i \neq 0$. And so, if there is a $z_i$ such that $z_i = 0$, then before the search, replace intervals $[z_{i-1}, z_i]$, $[z_i, z_{i+1}]$ with $[z_{i-1}, -\delta], [-\delta, \delta], [\delta, z_{i+1}]$ for $\delta$ small enough. It is clear that identifying $a_1$ to be within any of these three intervals would still allow for $\epsilon$-close estimation of $\mu(h^*)$. This modification means that we binary search over $k+2$ numbers. Either way, the search completes in $O(\log k)$ queries.

% The sample complexity needed to identify the interval is,
% $$\log \frac{1 - (-1)}{\min_{i \in [k]} z_{i+1} - z_i}$$

% \chicheng{$z_1, \ldots, z_{k+1}$ are all pre-computed, so we just need to find out $\max\cbr{i: z_i \leq a_i}$ using binary search over these $k+1$ numbers? This should only take $O(\log k)$ queries?} \note{I see, thanks for the pointer}

% It remains to lower bound $\min_{i \in [k]} z_{i+1} - z_i$. We have by Intermediate Value Theorem:
% \begin{align*}
%     \epsilon & = \Phi(\alpha z_{i+1} +1) - \Phi(\alpha z_i + 1) \\ 
%     & = \Phi'(\alpha(z_i + \lambda'(z_{i+1} - z_i)) + 1) (z_{i+1} - z_i) \\
%     & = \exp(-(\alpha(z_i + \lambda'(z_{i+1} - z_i)) + 1)^2 / 2) (z_{i+1} - z_i)
% \end{align*}
% \chicheng{Why don't we directly upper bound the exponential term by 1, so we have $\epsilon \leq z_{i+1} - z_i$?} \note{Oh good point}

% where we know that $\alpha(z_i + \lambda'(z_{i+1} - z_i)) + 1 \in [1 - \alpha, 1 + \alpha]$.

% We will argue that $\alpha = o(1)$. Suppose not, let $\alpha \geq C_2$ for some constant $C_2$. Then, $\Phi(1 + \alpha) - \Phi(1) \geq \Phi(1 + C_2) - \Phi(1) = \exp(-(1 + \lambda C_2)^2 / 2) C_2 = C_3$ for $\lambda \in [0,1]$ and some constant $C_3$. This is a contradiction since $o(1) = k\epsilon = \Phi(1 + \alpha) - \Phi(1 - \alpha) > \Phi(1 + \alpha) - \Phi(1) \geq C_3$.

% Thus, $\alpha = o(1)$. Using this, for any $i$,
% \begin{align*}
%     \epsilon & = \exp(-(\alpha(z_i + \lambda'(z_{i+1} - z_i)) + 1)^2 / 2) (z_{i+1} - z_i) \\
%     & \leq \exp(-(1 - \alpha)^2/ 2) (z_{i+1} - z_i) \\
%     & = C_1 (z_{i+1} - z_i)
% \end{align*}

% for some constant $C_1$. This means that, $z_{i+1} - z_i \geq \epsilon / C_1$ for all $i \in [k]$, and we have:
% $$\log \frac{2}{\min_{i \in [k]} z_{i+1} - z_i} \leq O(\log 1 / \epsilon)$$

\textbf{Active Learning Lower Bound:} To establish a lower bound, we will be making use of the following result from \cite{kulkarni1993active}:

\begin{theorem}
$O(\log |N(2\epsilon, \Hcal, \Dcal)|)$ queries are necessary by any active learning algorithm, randomized or deterministic, in order to learn a concept class $\Hcal$ with respect to distribution $\Dcal$, where $|N(2\epsilon, \Hcal, \Dcal)|$ is a minimal $2\epsilon-$covering of $\Hcal$ with respect to the disagreement metric.
\end{theorem}

It now suffices to provide a lower bound on the covering number (or the entropy of) $\Hcal = \{(a, 1): a \in \mathbb{R}^d, \|a\| = 1\}$. We will take $\Pr(x_A = 1) = 1/2$.

Our goal is to construct a $2 \cdot 4\epsilon-$packing of $\Hcal$ with respect to $\Pr(x_A = 0)$. This lower bounds the size of any $4\epsilon-$packing of $\Hcal$ wrt $\Dcal$, which lower bounds the size of (any) and the minimal $2\epsilon-$covering of $\Hcal$ under $\Dcal$.

\note{Find this $O(\frac{1}{\epsilon}^d)$ covering wrt $\ell_2$ on sphere in literature. Show that $\ell_2$ translates that: if $\theta(w_1, w_2) = \arccos(w_1 \cdot w_2) \leq 2\epsilon$.}

To do this, we will show that a random sample of $\Omega((1 / \epsilon)^d)$ $w$'s from the sphere will be a $8\epsilon-$packing with non-zero probability. This means that there must exist a packing of size $\Omega((1 / \epsilon)^d)$, which in turn bounds the size of any $2\epsilon-$covering.

We have that with \note{fill in} probability the sample of $\Omega((1 / \epsilon)^d)$ $a$'s will be such that any two $a, a'$ is s.t $\theta(a_1, a_2) \leq c\epsilon$ \note{fill in constant}. To finish, we will lower bound $\Pr_{x \sim N(0, I)}(a \cdot x + 1 \geq 0 \land a' \cdot x + 1 < 0)$.

%Using Theorem 2.8 of \url{https://www.cs.cornell.edu/jeh/book.pdf}, with nonzero probability, there exists a set of $n = \exp(d)$ unit norm vectors for which this holds pairwise. Then, we will show that for any $a, a'$ is s.t $|a \cdot a'| \leq \cos \theta$: $$\Pr_{x \sim N(0, I)}(a \cdot x + 1 \geq 0 \land a' \cdot x + 1 < 0) \geq 4\epsilon$$

For simplicity, for a pair of vectors $a, a'$, one can apply a rotation to map them to $a = (1, 0, 0, ...)$ and $a' = (\cos \theta, \sin \theta, 0, ...))$ while preserving inner product and thus $\Pr_{x \sim N(0, I)}(a \cdot x + 1 \geq 0 \land a' \cdot x + 1 < 0)$. Then, a subset of the disagreement region is: $x_1 \geq -1$ and $\cos \theta x_1 + \sin \theta x_2 + 1 < 0$.

Pictorially, this corresponds to the disagreement region formed by lines $x = -1$ and the line perpendicular to $y = (\cos \theta / \sin \theta) x$ passing through $(\cos \theta, \sin \theta)$. These two lines intersect at a point $O$ such that the line from this point to the origin bisect the angle between the x-axis and $y = \cos \theta / \sin \theta x$. From this, we get that $O = (-1, -\sin \theta / 2)$.

The disagreement region thus comprise of two regions of different density:
$$\int \int \exp(-1/2 ((u - 1)^2 + (u - \sin \theta / 2)^2)) du dv$$

over $u^2 + v^2 \leq R$ and $\theta(u,v) \in [\pi/2, \pi/2 + \theta] \cup [3\pi/2, 3\pi/2 + \theta]$.

Actually, consider the triangle formed by $O$, point $(-1, 1 - \sin \theta/2)$ and point $V$, $(-1-\tan \theta, 1)$. This is a subset of the disagreement region. By construction, it has area $1 /2 \tan \theta$ and each point in the triangle has density at least $\exp(-1/2((-1-\tan \theta)^2 + (-1)^2)) \geq \exp(-1/2(5))$, just by looking at the max absolute value of the x and y coordinates of points in this region. And so, we know the disagreement region probability is lower bounded by $\exp(-1/2(5)) 1/2 \tan \theta \approx 1/2 \exp(-1/2(5)) \theta$.

%We need $\sin \theta > 0$ %\note{account for this, mirror in rotation}:

% \begin{align*}
%     & \Pr_{x \sim N(0, I)}(a \cdot x + 1 \geq 0 \land a' \cdot x + 1 < 0) \\
%     & = 1 / 2\pi \int_{-1}^{\infty} \int_{-\infty}^{ \frac{-x_1}{\tan \theta} - \frac{1}{\sin \theta}} \exp(-1/2(x_1^2 + x_2^2)) d x_1 d x_2 \\
%     & = C \int_{-1}^{\infty} \Phi(\frac{-x_1}{\tan \theta} - \frac{1}{\sin \theta}) \exp(-1/2 x_1^2) dx_1
% \end{align*}
% which seems to give a constant lower bound on the probability of being in the disagreement region, e.g evaluating around $x_1 \in [-1, 1]$%...\note{come back to this, seems very loose}.


\end{proof}

%\note{+Active Learning lower bound using Packing result from Kulkarni, Mitter, Tsitsikli (their result is a lower bound on our setting). May use \url{https://www.cs.cornell.edu/jeh/book.pdf} Chapter 2 results on near-orthogonal vectors.}

\textbf{Discrete Setting:} $\Xcal$ is a set of $d$ points shattered by $\Hcal$. $\Dcal$ is uniform over $\Xcal$. 
\textbf{Proof:} Seem to be able to get a $2^{1 / \epsilon}$ covering by grouping $\Xcal$ into groups of $\epsilon |\Xcal|$ and models predict each group the same label.

\chicheng{
Examples where $\CC(\Hcal) \ll $ label complexity of active learning:
\begin{enumerate}
    \item $\mu(h) = $ constant, $\CC(\Hcal) = 0$
    \item $\Hcal = \cbr{ \sign(\inner{a}{x} + b): \|a\|_2 =1, b \in \RR}$ non-homogeneous linear classifiers,
    $x \mid x_A = 1 \sim N(\mu_1, I)$,  and $x \mid x_A = 0 \sim N(\mu_0, I)$,
    $\mu_1 = \alpha e_1$ ($\alpha > 0$), $\mu_0 = 0$,
    \[
    \PP(h^*(x) = +1 \mid x_A = 0)
    = 
    \Phi(b),
    \quad
    \PP(h^*(x) = +1 \mid x_A = 1)
    = 
    \Phi(a_1 \alpha + b)
    \]
    $|a_1| \leq 1$, exists suitable $\alpha$ DP $= \Phi(a_1 \alpha + b) - \Phi(b)$ as function of 
    $(a_1, b)$ lies in $[-2\epsilon, 2\epsilon]$.
    In other words,
    \[
    \min_{a,b} \Phi(a_1 \alpha + b) - \Phi(b) = -2\epsilon, 
    \max_{a,b} \Phi(a_1 \alpha + b) - \Phi(b) = +2\epsilon
    \]
    as a consequence,
    $\CC(\Hcal) > 0$.
    For auditing, it
    suffices to use $x = C e_1$ for large $C \geq \frac{1}{\epsilon^{10}}$ to check what sign $a_1$ is. Return estimate $\sign(a_1) \epsilon$.
    %\item 
    Tests: $x = 0, Ce_1, -Ce_1$. $x = 0$ gives sign of $b$. WLOG $\sign(b) = 1$, then if $x=-Ce_1$ has opposite label to $x = Ce_1$, then can tell the sign of $a_1$
    \begin{itemize}
        \item If $h^*(Ce_1) = +1$ and $h^*(-Ce_1) = -1$, then $a_1 > 0$
        \item If $h^*(Ce_1) = -1$ and $h^*(-Ce_1) = +1$, then $a_1 < 0$
        \item If $h^*(Ce_1) = +1$ and $h^*(-Ce_1) = +1$, $b / |a_1| > C$. Can we argue that $f(b) = \Phi(b(1 + \alpha a_1 / b)) - \Phi(b)$ is small?
        \[
        \approx \exp(-\frac{b^2}{2}) \cdot (\alpha a_1)
        \]
        Consider two cases:
        (1) $b \geq 10 \sqrt{\ln\frac{1}{\epsilon}}$. In this case, the above is at most $\epsilon^{10}$.
        (2) $b < 10 \sqrt{\ln\frac{1}{\epsilon}}$. In this case, $|a_1| \leq \frac{b}{C} \leq \frac{10 \sqrt{\ln\frac{1}{\epsilon}}}{C} \leq \epsilon^{10}$; in this case, the above is also at most $\epsilon^{10}$. 
        \\
        In contrast, for active learning, using existing distribution-dependent lower bounds (Kulkarni, Mitter, Tsitsiklis, Active learning with binary valued queries), we can show that active learning needs $\Omega(d \ln\frac{1}{\epsilon})$ label complexity. (TODO: work out the details)
    \end{itemize}
    \item Learn using $\Hcal = \{(a, 1): a \in \mathbb{R}^d, \|a\| = 1\}$. Pick $\alpha$ s.t DP ($= \Phi(a_1 \alpha + 1) - \Phi(1)$) $\in [-C_1 \epsilon, C_2\epsilon]$ where $C_1, C_2 \geq 3$ are absolute constants. Now figure out ranges of $a$ s.t the DP $\in [k\epsilon, (k+1)\epsilon]$ using binary search since DP is monotonic in $a_1$.
    More precisely, if $\abs{a_1} \leq \epsilon^{10}$, then $DP \leq \epsilon^{10}$.
    Given choice of $\alpha$ induces intervals $[z_1, z_2], (z_2, z_3]...$etc s.t if $a_1 \in (z_i, z_{i+1}] \Leftrightarrow DP \in [i \epsilon, (i + 1) \epsilon]$.
    Algorithm: searching for $a$ in $[z_1, z_k]$ to the precision of the minimal width of the interval
    $z_i$ is defined by: $\Phi(\alpha z_i +1) - \Phi(1) = i \epsilon$? 
    Assume $k \leq \frac{1}{10\epsilon}$. 
    Binary search: test if $a_1 > c$, deploy $-1 / c e_1 \rightarrow$ positive label. Binary search: $O(\log k)$? $O(k)$. 
    Find some value in $[z_1, z_k]$, just care about which interval $[z_i, z_{i+1}]$ $a_1$ is in
    \\
    We can show for every $i$, $C_3 \epsilon \geq \abs{z_{i+1} - z_i} \geq C_4 \epsilon$
    \item Same setting as before, but for $h^* = (w^*, b^*)$, $b^*$ is very large. Active learning is hard - we can possibly find a example similar the disjoint interval example in this setting, where we are likely to have $\Omega(1/\epsilon)$ label complexity lower bound (TODO: check the following papers about results on active learning non-homogeneous linear separator class:
    \url{http://www.cs.cmu.edu/~ninamf/papers/true-active-journal.pdf}\url{https://cseweb.ucsd.edu/~dasgupta/papers/sample.pdf} (linear separator in $\RR^3$)). Deterministic Auditing has a label complexity of $O(d)$?
    \end{enumerate}
}


%%%%%


\chicheng{Designing deterministic algorithms for auditing with $\tilde{O}(d \cdot  \polylog\frac1\epsilon)$ label complexity in this setting:
}

WLOG, $D_X = N(0, I)$
\begin{itemize}
    \item Key observation (corner cases): \begin{enumerate}
        \item If $b \geq \sqrt{\ln\frac1\epsilon}$, then $\mu(h^*) \geq 1-\epsilon$
        \item If $b \leq -\sqrt{\ln\frac1\epsilon}$, then $\mu(h^*) \leq \epsilon$
        \item If $b \in [-\epsilon, \epsilon]$, then $\abs{\mu(h^*) - \frac12} \leq \epsilon$
    \end{enumerate}
    \item Primitive 1: we can test whether $m_i = \frac{b}{a_i} \in [-M, M]$, by querying $M e_i$ and $-M e_i$ -- if they have opposite signs, it must be the case that $m_i \in [-M, M]$; otherwise, $m_i \notin [-M, M]$. 
    
    \item Primitive 2: suppose we know that $m_i = \frac{b}{a_i} \in [-M, M]$, then we can use binary search to obtain an estimate of it, $\hat{m}_i$, such that $\abs{ \hat{m}_i - m_i } \leq \zeta$, with label complexity $\log\frac{2M}{\zeta}$.
    \item Now, for algorithm design:
    \begin{enumerate}
        \item Use Primitive 1 for $M = \sqrt{d \ln\frac1\epsilon}$ at each coordinate to see if it is the case that for all $i$, $\abs{m_i} \geq \sqrt{d \ln\frac1\epsilon}$. If yes, as there exists at least one $i$ such that $|a_i|_2 \geq \frac{1}{\sqrt{d}}$, we must have $\abs{b} \geq \sqrt{\ln\frac1\epsilon}$. 
        In this case, we additionally query $0$ to get the sign of $b$; if $\sign(b) > 0$,
        $\mu(h^*) \geq 1-\epsilon$, we can output auditing estimate as $1$; otherwise, 
        $\mu(h^*) \leq \epsilon$, we output auditing estimate as $0$. Otherwise, go to the next case.
        \item We are in the case that there exists some $i_0$, $|m_{i_0}| \leq \sqrt{d\ln\frac1\epsilon}$. In this case, we first observe that
        \[
        \sum_{i=1}^d \frac{1}{m_i^2} 
        \geq 
        \frac{1}{m_{i_0}^2}
        \geq 
        \frac{1}{d \ln\frac1\epsilon}.
        \]
        
        %As $\| a \|_2 \leq 1$, we have $\abs{b} = m_{i_0} \cdot | a_{i_0} | \leq \sqrt{d\ln\frac1\epsilon}$. 
        Our goal is to provide estimate to $m_i$ for all $i$ -- call it $\hat{m}_i$, such that 
        $\abs{\frac{1}{(m_i)^2} - \frac{1}{(\hat{m}_i)^2}} \leq \xi$ (where $\xi$ is to be decided later). To this end, we use Primitive 1 with $|m_i| \geq  \sqrt{\frac1\xi}$.
        Consider two possible outcomes:
        \begin{enumerate}
            \item $|m_i| \geq  \sqrt{\frac1\xi}$. In this case, we set $\hat{m}_i = +\infty$, and therefore, we have $\abs{\frac{1}{(m_i)^2} - \frac{1}{(\hat{m}_i)^2}} \leq \xi$ holding.
            \item $|m_i| < \sqrt{\frac1\xi}$. In this case, we use Primitive 2 to obtain $\hat{m}_i$ such that $\abs{\hat{m}_i - m_i} \leq \zeta$ (where $\zeta \leq \frac{\epsilon}{2}$ is to be decided later). If $\abs{\hat{m}_i} \leq \epsilon$, we have that $\abs{m_i} \leq \epsilon + \zeta \leq 2\epsilon$, which implies that $\abs{b} \leq \epsilon$, and therefore $\abs{\mu(h^*) - \frac12} \leq \epsilon$ - we can output our auditing estimate as $\frac12$. Otherwise, $\hat{m_i} \geq \frac \epsilon 2$, and we have:
            \[
            \abs{ \frac{1}{(\hat{m}_i)^2}
            -
            \frac{1}{(m_i)^2}
            }
            \leq 
            \frac{\zeta}{\epsilon^3}
            \leq \xi
            \]
        \end{enumerate}
        In summary, in both cases, we have $\abs{ \frac{1}{(\hat{m}_i)^2}
            -
            \frac{1}{(m_i)^2}
            } \leq \xi$ holding for all $i$. Therefore,
        \[
        \abs{
        \sum_{i=1}^d \frac{1}{(\hat{m}_i)^2}
            -
        \sum_{i=1}^d \frac{1}{(m_i)^2}
        }
        \leq 
        d \xi 
        \]
        We set $\xi$ such that $d \xi \leq \frac{1}{2d \ln\frac1\epsilon}$; in this case, we have that 
        \[
        \abs{
        \sqrt{
        \frac1 {\sum_{i=1}^d \frac{1}{(\hat{m}_i)^2} } }
            -
        \sqrt{
        \frac 1 {
        \sum_{i=1}^d \frac{1}{(m_i)^2}
        }} }
        \leq 
        d \xi \cdot (2d \ln\frac{1}{\epsilon})^{\frac{3}{2}} 
        \leq 
        \epsilon,
        \]
        with appropriate setting of $\xi$. In this case, we define our estimate of $|b|$, $\hat{l} = \sqrt{
        \frac1 {\sum_{i=1}^d \frac{1}{(\hat{m}_i)^2} } }$, which is $\epsilon$-close to $\sqrt{\frac 1 {
        \sum_{i=1}^d \frac{1}{(m_i)^2}
        }} = |b|$. Again, we additionally query $0$ to get the sign of $b$, so that we obtain $\hat{b}$ that is $\epsilon$-close to $b$. Our auditing estimate in this case is $\Phi(\hat{b})$, which is $\epsilon$-close to $\Phi(b)$ by the Lipschitzness of $\Phi$. 
    \end{enumerate}
\end{itemize}

\chicheng{initially, I thought this can be a good example that separates the complexity from auditing to active learning, as I conjecture that active learning has a label complexity at least $\Omega(\frac1\epsilon)$. (If this were true, then when $d \ll \frac1\epsilon$, auditing's label complexity $\tilde{O}(d)$ is much smaller than active learning's.)
However, this is likely not the case. The key issue is that the above algorithm almost also works for active learning: in case 1, we can just output all $+1$ classifier or all $-1$ classifier; in case 2, we first use the above algorithm to obtain an $O(\epsilon)$-accurate estimate of $b$, and use the above guarantee that 
$\abs{ \frac{1}{(\hat{m}_i)^2}-\frac{1}{(m_i)^2}} \leq \xi$ to estimate all $a_i$'s to a precision of $O(\frac{\epsilon}{\sqrt{d}})$. So active learning also has a label complexity of $\tilde{O}(d)$. 
}
\chicheng{Some useful tools for learning non-homogeneous linear spearators: \url{http://www.cs.cmu.edu/~ninamf/papers/true-active-journal.pdf}}
